Structured Outdoor Architecture Reconstruction by Exploration and Classification

This paper presents an explore-and-classify framework for structured architectural reconstruction from an aerial image. Starting from a potentially imperfect building reconstruction by an existing algorithm, our approach 1) explores the space of building models by modifying the reconstruction via heuristic actions; 2) learns to classify the correctness of building models while generating classification labels based on the ground-truth, and 3) repeat. At test time, we iterate exploration and classification, seeking for a result with the best classification score. We evaluate the approach using initial reconstructions by two baselines and two state-of-the-art reconstruction algorithms. Qualitative and quantitative evaluations demonstrate that our approach consistently improves the reconstruction quality from every initial reconstruction.

==> sections/03-rl.tex <==
\section{Relationship to Reinforcement Learning} \label{section:rl}
%Our system is a special case of q-learning, whose general formula is
%\begin{eqnarray}
%Q(s,a) = \mathbb{E}_{s^\prime \sim \mathcal{E}} \left[R(s,a) + \gamma \underset{a^\prime}{\text{max}}Q(s^\prime, a^\prime) | s,a\right].
%\label{eq:tdrl}
%\end{eqnarray}

Our system is a special case of temporal difference reinforcement learning (TD-RL) for a state value function, whose general formula is
\begin{eqnarray}
V^{\pi}(s) = \mathbb{E}_{\pi} \left[R(s,a) + \gamma  V^{\pi}(s^\prime)| s\right].
\label{eq:td-v}
\end{eqnarray}
$s$ is the current state and $s^\prime$ is the next state after an action $a$ with reward $R(s,a)$. $\gamma$ and $V$ denote a discount factor and a state value function. $\pi$ is the policy. Intuitively, our classifiers evaluate goodness of a reconstruction and are equivalent to value function. Classification labels are based on ground-truth and are equivalent to reward. Three specializations reduce this TD-RL formulation into our approach.
%value function estimation to our training.

\vspace{0.1cm}
\noindent $\bullet$
The first specialization is $\gamma$=0, ignoring future rewards, which would be important for adversarial tasks such as a Chinese game of Go~\cite{silver2017mastering} or a strategy game like StarCraft~\cite{vinyals2019alphastar}. Geometry reconstruction is a stable process and we trust the current reward 100\%. This reduces Eq.~\ref{eq:td-v} to $V^{\pi}(s) = \mathbb{E}_{\pi} \left[R(s,a)| s\right]$.%$Q(s, a) = \mathbb{E}_{s^\prime \sim \mathcal{E}} [R(s,a) | s,a] = R(s,a)$.%$V(s)=r$, which means that our system is effectively estimating the state value function of the current graph while disregarding all future rewards. 

\noindent
$\bullet$ The second specialization is the assumption that the reward solely depends on the state, which 
%is independent of action. Classification label defined in section~\ref{sec:classifiers} only depends on the goodness of the current state. This
allows us to rewrite Eq.~\ref{eq:td-v} as $V^{\pi}(s) = \mathbb{E}_{\pi} \left[R(s)| s\right]$. Since the term does not depend on actions, we remove the expectation over policy $\pi$ and further simplify it as $V(s) = R(s)$.
%, revealing our approach: setting the labels directly as the classifier output.

\noindent
$\bullet$ The third specialization is the design of a value function, which is typically a single function evaluating the goodness of an entire state~\cite{ellis2019write,lin2020modeling}.
%most critical: the design of value function. 
We use a set of classifiers over local primitives of varying degrees (i.e., junctions, edges, and regions).
%as opposed to a single value function for entire structure.
The reward is also broken down to local primitives, and we have $V(\tilde{s})=R(\tilde{s})$ for each geometric primitive $\tilde{s}$, which exactly matches our formulation in Sec.~\ref{sec:classifiers}.



